Reduction of Copper Oxide by Formic Acid an ab-initio study

Four cluster models for a copper(I)oxide (111) surface have been designed, of which three were studied with respect to their applicability in density functional calculations in the general gradient approximation. Formic acid adsorption on these systems was modelled and yielded four different adsorption structures, of which two were found to have a high adsorption energy. The energetically most favourable adsorption structure was further investigated with respect to its decomposition and a few reactions with adsorbed H and OH species using synchronous transit methods to estimate reaction barriers and single point energy calculations for the reaction energy.

==> conclusion/conclusion.tex <==
\chapter{Conclusion}

yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
\begin{center}
yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
yaddayaddayadda
\end{center}



